Effect of Particle Size on the Suction Mechanism in Granular Grippers

Granular grippers are highly adaptable end-effectors that exploit the reversible jamming transition of granular materials to hold and manipulate objects. Their holding force comes from the combination of three mechanisms: frictional forces, geometrical constraints, and suction effects. In this work, we experimentally study the effect of particle size on the suction mechanism. Through X-ray computed tomography, we show that small particles (average diameter d = 120 micrometers) achieve higher conformation around the object than larger particles (d = 4mm), thus allowing the formation of air-tight seals. When the gripper is pulled off, mimicking lifting of an object, vacuum pressure is generated in the sealed cavity at the interface gripper--object. If the particles used as filling material are too large, the gripper does not conform closely around the object, leaving gaps between the gripper's membrane and the object. These gaps prevent the formation of sealed vacuum cavities between the object and the gripper and in turn hinder the suction mechanism from operating.

==> images-setup/Experimental-Setup-corrected.tex <==
\begin{tikzpicture}

\node[] (setup)  at (0, 0) {\includegraphics[width=0.65\linewidth, trim=12cm 1.3cm 12cm 2.5cm, clip]{images-setup/Experimental-Setup-corrected3.png}};

%\node[left=2mm of setup.187, anchor=east, align=flush right] (sensor) 
%{load cell};
%\node[right=0.18*\linewidth of sensor] (sensorPt) {};
%\draw[-{Circle[open]}, thick](sensor.east)--(sensorPt);

\node[above=-4mm of setup.95] (vac1) {};
\node[above=8mm of setup.95] (vac2) {};
\draw[-stealth, ultra thick](vac1)--(vac2) node [midway, right=1mm, yshift=-2pt]{vacuum};

\node[right=2mm of setup.12, anchor=west, text width=3.5cm] (membrane) {membrane\\ filled with particles};
\node[left=41mm of membrane] (membranePt) {};
\draw[white, ultra thick](membrane.west)--(membranePt);
\draw[-{Circle[fill=white]}, thick](membrane.west)--(membranePt);

\node[right=2mm of setup.-6, anchor=west] (object) {object};
\node[left=47mm of object] (objectPt) {};
\draw[ultra thick, white](object.west)--(objectPt);
\draw[-{Circle[fill=white]}, thick](object.west)--(objectPt);

\node[right=2mm of setup.-13, anchor=west] (tunnel) {vacuum test tunnel};
\node[left=48mm of tunnel] (tunnelPt) {};
\draw[ultra thick, white](tunnel.west)--(tunnelPt.center);
\draw[-{Circle[fill=white]}, thick](tunnel.west)--(tunnelPt.center);

\node[right=2mm of setup.-29, anchor=west] (loadcell) {load cell};
\node[left=38mm of loadcell] (loadcellPt) {};
\draw[ultra thick, white](loadcell.west)--(loadcellPt.center);
\draw[-{Circle[fill=white]}, thick](loadcell.west)--(loadcellPt.center);

\node[right=2mm of setup.-38, anchor=west] (zstage) {$z$-stage};
\node[below=24mm of setup.center, xshift=-4mm] (zstagePt) {};
\node[left=36mm of zstage, yshift=2pt] (zstagePtmid) {};
\draw[ultra thick, white](zstage.west)--(zstagePtmid.center)--(zstagePt.center); 
\draw[-{Circle[fill=white]}, thick](zstage.west)--(zstagePtmid.center)--(zstagePt.center); 

\draw[stealth-, ultra thick](-1.6,-1.47)--(-0.6,-1.47) node [midway, above]{$p$};


\end{tikzpicture}
